Recurrent Neural Networks For Accurate RSSI Indoor Localization

This paper proposes recurrent neuron networks (RNNs) for a fingerprinting indoor localization using WiFi. Instead of locating user's position one at a time as in the cases of conventional algorithms, our RNN solution aims at trajectory positioning and takes into account the relation among the received signal strength indicator (RSSI) measurements in a trajectory. Furthermore, a weighted average filter is proposed for both input RSSI data and sequential output locations to enhance the accuracy among the temporal fluctuations of RSSI. The results using different types of RNN including vanilla RNN, long short-term memory (LSTM), gated recurrent unit (GRU) and bidirectional LSTM (BiLSTM) are presented. On-site experiments demonstrate that the proposed structure achieves an average localization error of $0.75$ m with $80\%$ of the errors under $1$ m, which outperforms the conventional KNN algorithms and probabilistic algorithms by approximately $30\%$ under the same test environment.

==> macros.tex <==

\makeatletter
\def\argmin{\mathop{\operator@font argmin}}
\def\argmax{\mathop{\operator@font argmax}}
\makeatother

\newcommand{\half}{\frac{1}{2}}
\newcommand{\CM}{{\cC\!\cM}}
\newcommand{\ZCM}{{\mbox{ZCM}}}
\newcommand{\Rp}{{R^\prime}}
\newcommand{\Rpp}{{R^{\prime \prime}}}
\newcommand{\dist}{\mbox{\rm dist}}

\def\fracN{\textstyle\frac{1}{N}}

\newcommand{\var}{\mbox{\rm var}}
\newcommand{\cov}{\mbox{\rm cov}}
\newcommand{\cum}{\mbox{\rm cum}}
\newcommand{\real}{\mbox{\rm real}}
\newcommand{\imag}{\mbox{\rm imag}}
\renewcommand{\Re}{\mbox{\rm Re}}
\renewcommand{\Im}{\mbox{\rm Im}}
\newcommand{\eig}{\mbox{\rm eig}}
\newcommand{\diag}{\mbox{\rm diag}}
\newcommand{\spann}{\mbox{\rm span}}
\newcommand{\rank}{\mbox{\rm rank}}
\newcommand{\Null}{\mbox{\rm Null}}
%\newcommand{\argmin}{\mbox{\rm arg}\min}
\newcommand{\Tr}{\mbox{\rm Tr}}
\newcommand{\tr}{\mbox{\rm tr}}
\newcommand{\dimm}{\mbox{\rm dim }}
\newcommand{\sdim}{\mbox{\rm s-dim }}
\newcommand{\unvec}{\mbox{\rm unvec}}
\newcommand{\vect}{\mbox{\rm vec}}
\newcommand{\rvec}{\mbox{\rm vecr}}
\newcommand{\unvect}{{\vect}^{-1}}
\newcommand{\vech}{\mbox{\rm vech}}
\newcommand{\unvech}{{\vech}^{-1}}
\newcommand{\range}{\mbox{\rm ran}}
\newcommand{\row}{\mbox{\rm row}}
\newcommand{\col}{\mbox{\rm col}}
\newcommand{\sign}{\mbox{\rm sign}}
\newcommand{\cond}{\mbox{\rm cond}}
\newcommand{\suchthat}{\hspace{1cm}\mbox{\rm s.t.}\hspace{.5cm}}
\newcommand{\GE}{{\rm GE}}
\newcommand{\SINR}{\mbox{\rm SINR}}
\newcommand{\INSR}{\mbox{\rm INSR}}
\newcommand{\SIR}{\mbox{\rm SIR}}
\newcommand{\SNR}{\mbox{\rm SNR}}
\newcommand{\AsN}{\mbox{{\rm As}\cN}}

\newcommand{\dr}{\ensuremath{\mathrm{d}}}

\def\cf{{cf.\ }}
\def\viz{{viz.\ }}
\def\etal{{et al.\ }}
\def\eg{{e.g.,\ }}
\def\ie{{i.e.,\ }}

\def\bm#1{\mbox{\boldmath $#1$}}
\newcommand{\balpha}{{\bm\alpha}}
\newcommand{\btau}{{\bm\tau}}
\newcommand{\bbeta}{{\bm\beta}}

\newcommand{\bea}{\begin{array}}
\newcommand{\ena}{\end{array}}
%
\newcommand{\beq}{\begin{equation}}
\newcommand{\enq}{\end{equation}}

\newcommand{\beqa}{\begin{eqnarray}}
\newcommand{\enqa}{\end{eqnarray}}

\newcommand{\beqan}{\begin{eqnarray*}}
\newcommand{\enqan}{\end{eqnarray*}}

\newcommand{\AL}{\begin{enumerate}}
\newcommand{\ALE}{\end{enumerate}}


\newcommand{\cA}{\ensuremath{\mathcal{A}}}
\newcommand{\cB}{\ensuremath{\mathcal{B}}}
\newcommand{\cC}{\ensuremath{\mathcal{C}}}
\newcommand{\cD}{\ensuremath{\mathcal{D}}}
\newcommand{\cE}{\ensuremath{\mathcal{E}}}
\newcommand{\cH}{\ensuremath{\mathcal{H}}}
\newcommand{\cI}{\ensuremath{\mathcal{I}}}
\newcommand{\cK}{\ensuremath{\mathcal{K}}}
\newcommand{\cL}{\ensuremath{\mathcal{L}}}
\newcommand{\cM}{\ensuremath{\mathcal{M}}}
\newcommand{\cN}{\ensuremath{\mathcal{N}}}
\newcommand{\cO}{\ensuremath{\mathcal{O}}}
\newcommand{\cP}{\ensuremath{\mathcal{P}}}
\newcommand{\cR}{\ensuremath{\mathcal{R}}}
\newcommand{\cS}{\ensuremath{\mathcal{S}}}
\newcommand{\cT}{\ensuremath{\mathcal{T}}}
\newcommand{\cU}{\ensuremath{\mathcal{U}}}
\newcommand{\cX}{\ensuremath{\mathcal{X}}}
\newcommand{\cZ}{\ensuremath{\mathcal{Z}}}
\newcommand{\cJ}{\ensuremath{\mathcal{J}}}


\newcommand{\rH}{^{ \raisebox{1pt}{$\rm \scriptscriptstyle H$}}}
%\newcommand{\rH}{^{*}}
\newcommand{\rT}{^{ \raisebox{1.2pt}{$\rm \scriptscriptstyle T$}}}
\newcommand{\rF}{_{ \raisebox{-1pt}{$\rm \scriptstyle F$}}}
\newcommand{\rE}{{\rm E}}

\newcommand{\Vn}{\Va^{\perp}}
\newcommand{\Un}{\Ua^{\perp}}
\newcommand{\bVn}{\bVa^{\perp}}
\newcommand{\bUn}{\bUa^{\perp}}
%\newcommand{\VnH}{\Va^{\perp{\rm\scriptscriptstyle *}}}
%\newcommand{\UnH}{\Ua^{\perp{\rm\scriptscriptstyle *}}}
\newcommand{\VnH}{\Va^{\perp *}}
\newcommand{\bVnH}{\bVa^{\perp *}}
\newcommand{\UnH}{\Ua^{\perp *}}
\newcommand{\bUnH}{\bUa^{\perp *}}
\newcommand{\sk}{\sigma_{d+1}}
\newcommand{\vk}{\bv_{d+1}}
\newcommand{\uk}{\bu_{d+1}}
\newcommand{\ukz}{u_{d+1}(z)}
\newcommand{\Ls}{\Lambda_s}
\newcommand{\Ln}{\Lambda_n}
\newcommand{\Lo}{\tilde{\Lambda}}
\newcommand{\Loh}{\tilde{\Lambda}^{1/2}}
\newcommand{\Las}{\hat{\Lambda}_s}
\newcommand{\Wh}{W^{1/2}}
\newcommand{\bRopt}{\bR^{\mbox{\scriptsize opt}}}
\newcommand{\Gammaopt}{\Gamma^{\mbox{\scriptsize opt}}}
\newcommand{\bGammaopt}{\bGamma^{\mbox{\scriptsize opt}}}
\newcommand{\Wlo}{W_{1,\mbox{\scriptsize opt}}}
 

% anti-diagonal dots
\def\addots{\mathinner{
    \mkern1mu\raise0pt\vbox{\kern7pt\hbox{.}}
    \mkern2mu\raise4pt\hbox{.}
    \mkern2mu\raise7pt\hbox{.}
    \mkern1mu}}

% steep diagonal dots
\def\sddots{\mathinner{
    \mkern.8mu\raise7pt\hbox{.}
    \mkern.8mu\raise4pt\hbox{.}
    \mkern.8mu\raise0pt\vbox{\kern7pt\hbox{.}}
    \mkern1mu}}

% steep anti-diagonal dots
\def\saddots{\mathinner{
    \mkern.2mu\raise0pt\vbox{\kern7pt\hbox{.}}
    \mkern.2mu\raise4pt\hbox{.}
    \mkern.2mu\raise7pt\hbox{.}
    \mkern1mu}}


\newcommand{\cHt}{{\tilde{\cal H}}}


\newcommand{\ba}{{\ensuremath{\mathbf{a}}}}
\newcommand{\bb}{{\ensuremath{\mathbf{b}}}}
\newcommand{\bc}{{\ensuremath{\mathbf{c}}}}
\newcommand{\bd}{{\ensuremath{\mathbf{d}}}}
\newcommand{\be}{{\ensuremath{\mathbf{e}}}}
\newcommand{\bff}{{\ensuremath{\mathbf{f}}}}
\newcommand{\bg}{{\ensuremath{\mathbf{g}}}}
\newcommand{\bh}{{\ensuremath{\mathbf{h}}}}
\newcommand{\bj}{{\ensuremath{\mathbf{h}}}}
\newcommand{\bn}{{\ensuremath{\mathbf{n}}}}
\newcommand{\bp}{{\ensuremath{\mathbf{p}}}}
\newcommand{\bpa}{{\ensuremath{\mathbf{\hat{p}}}}}
\newcommand{\bq}{{\ensuremath{\mathbf{q}}}}
\newcommand{\br}{{\ensuremath{\mathbf{r}}}}
\newcommand{\bs}{{\ensuremath{\mathbf{s}}}}
\newcommand{\bt}{{\ensuremath{\mathbf{t}}}}
\newcommand{\bu}{{\ensuremath{\mathbf{u}}}}
\newcommand{\bv}{{\ensuremath{\mathbf{v}}}}
\newcommand{\bw}{{\ensuremath{\mathbf{w}}}}
\newcommand{\bx}{{\ensuremath{\mathbf{x}}}}
\newcommand{\by}{{\ensuremath{\mathbf{y}}}}
\newcommand{\bz}{{\ensuremath{\mathbf{z}}}}

\newcommand{\bphi}{{\ensuremath{\mathbf{\phi}}}}

\newcommand{\bA}{{\ensuremath{\mathbf{A}}}}
\newcommand{\bB}{{\ensuremath{\mathbf{B}}}}
\newcommand{\bC}{{\ensuremath{\mathbf{C}}}}
\newcommand{\bD}{{\ensuremath{\mathbf{D}}}}
\newcommand{\bE}{{\ensuremath{\mathbf{E}}}}
\newcommand{\bF}{{\ensuremath{\mathbf{F}}}}
\newcommand{\bG}{{\ensuremath{\mathbf{G}}}}
\newcommand{\bH}{{\ensuremath{\mathbf{H}}}}
\newcommand{\bI}{{\ensuremath{\mathbf{I}}}}
\newcommand{\bJ}{{\ensuremath{\mathbf{J}}}}
\newcommand{\bK}{{\ensuremath{\mathbf{K}}}}
\newcommand{\bL}{{\ensuremath{\mathbf{L}}}}
\newcommand{\bM}{{\ensuremath{\mathbf{M}}}}
\newcommand{\bN}{{\ensuremath{\mathbf{N}}}}
\newcommand{\bO}{{\ensuremath{\mathbf{O}}}}
\newcommand{\bP}{{\ensuremath{\mathbf{P}}}}
\newcommand{\bQ}{{\ensuremath{\mathbf{Q}}}}
\newcommand{\bR}{{\ensuremath{\mathbf{R}}}}
\newcommand{\mR}{{\ensuremath{\mathbf{R}}}}
\newcommand{\mX}{{\ensuremath{\mathbf{X}}}}
\newcommand{\bS}{{\ensuremath{\mathbf{S}}}}
\newcommand{\bT}{{\ensuremath{\mathbf{T}}}}
\newcommand{\bU}{{\ensuremath{\mathbf{U}}}}
\newcommand{\bV}{{\ensuremath{\mathbf{V}}}}
\newcommand{\bW}{{\ensuremath{\mathbf{W}}}}
\newcommand{\bX}{{\ensuremath{\mathbf{X}}}}
\newcommand{\bY}{{\ensuremath{\mathbf{Y}}}}
\newcommand{\bZ}{{\ensuremath{\mathbf{Z}}}}


\newcommand{\da}{\ensuremath{\mathbf{\hat{d}}}}
\newcommand{\sa}{\ensuremath{\mathbf{\hat{s}}}}
\newcommand{\ea}{\ensuremath{\mathbf{\hat{e}}}}
\newcommand{\xa}{\ensuremath{\mathbf{\hat{x}}}}
\newcommand{\ya}{\ensuremath{\mathbf{\hat{y}}}}

\newcommand{\Aa}{\hat{A}}
\newcommand{\Ca}{\hat{C}}
\newcommand{\Ea}{\hat{E}}
\newcommand{\Ha}{\hat{H}}
\newcommand{\Lah}{\hat{\Lambda}}
\newcommand{\Ma}{\hat{M}}
\newcommand{\Na}{\hat{N}}
\newcommand{\Pa}{\hat{P}}
\newcommand{\Qa}{\hat{Q}}
\newcommand{\Ra}{\hat{R}}
\newcommand{\Sa}{\hat{\Sigma}}
\newcommand{\Sn}{\hat{\Sigma}^\perp}
\newcommand{\Ta}{\hat{T}}
\newcommand{\Ua}{\hat{U}}
\newcommand{\Va}{\hat{V}}
\newcommand{\Xa}{\hat{X}}
\newcommand{\Ya}{\hat{Y}}
\newcommand{\Za}{\hat{Z}}
\newcommand{\ua}{\hat{u}}

\newcommand{\bAa}{\ensuremath{\mathbf{\hat{A}}}}
\newcommand{\bCa}{\ensuremath{\mathbf{\hat{C}}}}
\newcommand{\bEa}{\ensuremath{\mathbf{\hat{E}}}}
\newcommand{\bHa}{\ensuremath{\mathbf{\hat{H}}}}
%\newcommand{\bLah}{\ensuremath{\mathbf{\hat{\bLambda}}}}
\newcommand{\bMa}{\ensuremath{\mathbf{\hat{M}}}}
\newcommand{\bNa}{\ensuremath{\mathbf{\hat{N}}}}
\newcommand{\bPa}{\ensuremath{\mathbf{\hat{P}}}}
\newcommand{\bQa}{\ensuremath{\mathbf{\hat{Q}}}}
\newcommand{\bRa}{\ensuremath{\mathbf{\hat{R}}}}
%\newcommand{\bSa}{\hat{\bSigma}}
\newcommand{\bSn}{{\bSigma}^\perp}
\newcommand{\bTa}{\ensuremath{\mathbf{\hat{T}}}}
\newcommand{\bUa}{\ensuremath{\mathbf{\hat{U}}}}
\newcommand{\bVa}{\ensuremath{\mathbf{\hat{V}}}}
\newcommand{\bWa}{\ensuremath{\mathbf{\hat{W}}}}
\newcommand{\bXa}{\ensuremath{\mathbf{\hat{X}}}}
\newcommand{\bYa}{\ensuremath{\mathbf{\hat{Y}}}}
\newcommand{\bZa}{\ensuremath{\mathbf{\hat{Z}}}}

\newcommand{\baa}{\ensuremath{\mathbf{\hat{a}}}}
\newcommand{\bua}{\ensuremath{\mathbf{\hat{u}}}}
\newcommand{\bta}{\ensuremath{\mathbf{\hat{t}}}}
\newcommand{\btac}{\ensuremath{\bar{\mathbf{\hat{t}}}}}
\newcommand{\bwa}{\ensuremath{\mathbf{\hat{w}}}}
\newcommand{\bya}{\ensuremath{\mathbf{\hat{y}}}}

% bar denotes conjugate
% tilde denotes noise
\newcommand{\Ac}{\bar{A}}
\newcommand{\Mc}{\bar{M}}
\newcommand{\Vc}{\bar{V}}
\newcommand{\Uc}{\bar{U}}
\newcommand{\Wc}{\bar{W}}
\newcommand{\Xtc}{\bar{\tilde{X}}}
\newcommand{\btc}{\bar{{\bf t}}}
\newcommand{\bat}{\tilde{{\bf a}}}
\newcommand{\bxt}{\tilde{{\bf x}}}
\newcommand{\bpt}{\tilde{{\bf p}}}
\newcommand{\xt}{\tilde{{\bf x}}}
\newcommand{\xtc}{\bar{\tilde{{\bf x}}}}
\newcommand{\Gt}{\tilde{G}}
\newcommand{\Pt}{\tilde{P}}
\newcommand{\Kt}{\tilde{K}}
\newcommand{\Xt}{\tilde{X}}
\newcommand{\Rt}{\tilde{R}}
\newcommand{\Ct}{\tilde{C}}
\newcommand{\Et}{\tilde{E}}

\newcommand{\bAc}{\ensuremath{\mathbf{\bar{A}}}}
\newcommand{\bCc}{\ensuremath{\mathbf{\bar{C}}}}
\newcommand{\bDc}{\ensuremath{\mathbf{\bar{D}}}}
\newcommand{\bMc}{\ensuremath{\mathbf{\bar{M}}}}
\newcommand{\bRc}{\ensuremath{\mathbf{\bar{R}}}}
\newcommand{\bTc}{\ensuremath{\mathbf{\bar{T}}}}
\newcommand{\bVc}{\ensuremath{\mathbf{\bar{V}}}}
\newcommand{\bUc}{\ensuremath{\mathbf{\bar{U}}}}
\newcommand{\bWc}{\ensuremath{\mathbf{\bar{W}}}}
\newcommand{\bZc}{\ensuremath{\mathbf{\bar{Z}}}}
\newcommand{\bXtc}{\ensuremath{\mathbf{\bar{\tilde{X}}}}}
\newcommand{\bGt}{\ensuremath{\mathbf{\tilde{G}}}}
\newcommand{\bPt}{\ensuremath{\mathbf{\tilde{P}}}}
\newcommand{\bKt}{\ensuremath{\mathbf{\tilde{K}}}}
\newcommand{\bXt}{\ensuremath{\mathbf{\tilde{X}}}}
\newcommand{\bRt}{\ensuremath{\mathbf{\tilde{R}}}}
\newcommand{\bCt}{\ensuremath{\mathbf{\tilde{C}}}}
\newcommand{\bEt}{\ensuremath{\mathbf{\tilde{E}}}}

\newcommand{\Xac}{\bar{\hat{X}}}
\newcommand{\Xc}{\bar{X}}
\newcommand{\bXac}{\ensuremath{\mathbf{\bar{\hat{X}}}}}
\newcommand{\bXc}{\ensuremath{\mathbf{\bar{X}}}}

\newcommand{\uc}{\bar{u}}
\newcommand{\buc}{\bar{\bu}}
\newcommand{\ucv}{\undertilde{\bar{u}}}
\newcommand{\bucv}{\undertilde{\bar{\bu}}}
\newcommand{\bUcv}{\undertilde{\bUc}}
\newcommand{\bLambdav}{\undertilde{\bLambda}}

\newcommand{\xc}{\bar{x}}
\newcommand{\sbar}{\bar{s}}
\newcommand{\bac}{\ensuremath{\mathbf{\bar{a}}}}
\newcommand{\bdc}{\ensuremath{\mathbf{\bar{d}}}}
\newcommand{\bec}{\ensuremath{\mathbf{\bar{e}}}}
\newcommand{\bgc}{\ensuremath{\mathbf{\bar{g}}}}
\newcommand{\bnc}{\ensuremath{\mathbf{\bar{n}}}}
\newcommand{\bxc}{\ensuremath{\mathbf{\bar{x}}}}
\newcommand{\bwc}{\ensuremath{\mathbf{\bar{w}}}}
\newcommand{\bwt}{\ensuremath{\mathbf{\tilde{t}}}}
\newcommand{\bst}{\ensuremath{\mathbf{\tilde{s}}}}
\newcommand{\bsc}{\ensuremath{\mathbf{\bar{s}}}}
\newcommand{\bzc}{\ensuremath{\mathbf{\bar{z}}}}

% dots
\newcommand{\bIdot}{\ensuremath{\mathbf{\dot{I}}}}

% whitened denoted by underline
\def\baw{\underline{\ba}}
\def\bacw{\underline{\bac}}
\def\baww{\underline{\underline{\ba}}}
\def\bacww{\underline{\underline{\bac}}}
\def\Aw{\underline{A}}
\def\Acw{\underline{\Ac}}
\def\Cw{\underline{C}}
\def\Ctw{\underline{\Ct}}
\def\Nw{\underline{N}}
\def\Gw{\underline{G}}
\def\Pw{\underline{P}}
\def\Rw{\underline{R}}
\def\Ww{\underline{W}}
\def\Xw{\underline{X}}
\def\Xtw{\underline{\Xt}}
\def\bxtw{\underline{\bxt}}
\def\bxcw{\underline{\bxc}}
\def\xtw{\underline{\bxt}}
\def\baw{\underline{\ba}}
\def\bxw{\underline{\bx}}
\def\bww{\underline{\bw}}
\def\byw{\underline{\by}}
\newcommand{\Gtw}{\underline{\Gt}}
\newcommand{\Ptw}{\underline{\Pt}}
\newcommand{\Rtw}{\underline{\Rt}}
\def\Xww{\underline{\underline{X}}}
\def\Xtww{\underline{\underline{\Xt}}}
\def\Ctww{\underline{\underline{\Ct}}}
\def\Aww{\underline{\underline{A}}}
\def\Acww{\underline{\underline{\Ac}}}
\def\Nww{\underline{\underline{N}}}
\def\Rtww{\underline{\underline{\Rt}}}
\def\Ktww{\underline{\underline{\Kt}}}
\def\Kww{\underline{\underline{K}}}

\def\bAw{\underline{\bA}}
\def\bAcw{\underline{\bAc}}
\def\bCw{\underline{\bC}}
\def\bCtw{\underline{\bCt}}
\def\bCaw{\underline{\bCa}}
\def\bNw{\underline{\bN}}
\def\bGw{\underline{\bG}}
\def\bPw{\underline{\bP}}
\def\bRw{\underline{\bR}}
\def\bWw{\underline{\bW}}
\def\bXw{\underline{\bX}}
\def\bXcw{\underline{\bXc}}
\def\bXwc{\underline{\bXc}}
\def\bXtw{\underline{\bXt}}
\def\bYw{\underline{\bY}}
\newcommand{\bGtw}{\underline{\bGt}}
\newcommand{\bPtw}{\underline{\bPt}}
\newcommand{\bRtw}{\underline{\bRt}}
\def\bXww{\underline{\underline{\bX}}}
\def\bXtww{\underline{\underline{\bXt}}}
\def\bCtww{\underline{\underline{\bCt}}}
\def\bAaw{\underline{\bAa}}
\def\bAww{\underline{\underline{\bA}}}
\def\bAcww{\underline{\underline{\bAc}}}
\def\bNww{\underline{\underline{\bN}}}
\def\bRtww{\underline{\underline{\bRt}}}
\def\bKtww{\underline{\underline{\bKt}}}
\def\bKww{\underline{\underline{\bK}}}

% composite denoted by undertilde
%\usepackage{amsmath}

% copied from amsmath: (don't load it all because destroys bold Sigma...)
\makeatletter
\def\setboxz@h{\setbox\z@\hbox}
\def\wdz@{\wd\z@}
\def\boxz@{\box\z@}
\def\underset#1#2{\binrel@{#2}%
  \binrel@@{\mathop{\kern\z@#2}\limits_{#1}}}
\def\binrel@#1{\begingroup
  \setboxz@h{\thinmuskip0mu
    \medmuskip\m@ne mu\thickmuskip\@ne mu
    \setbox\tw@\hbox{$#1\m@th$}\kern-\wd\tw@
    ${}#1{}\m@th$}%
  \edef\@tempa{\endgroup\let\noexpand\binrel@@
    \ifdim\wdz@<\z@ \mathbin
    \else\ifdim\wdz@>\z@ \mathrel
    \else \relax\fi\fi}%
  \@tempa
}
\let\binrel@@\relax%
\makeatother

% best choice:
\def\undertilde#1{\smash{\underset{^{\mbox{\~{}}}}{#1}}\vphantom{#1}}


\newcommand{\Av}{\ensuremath{\undertilde{A}}}
\newcommand{\bAv}{\ensuremath{\mathbf{\undertilde{\bA}}}}
\newcommand{\Dv}{\ensuremath{\undertilde{D}}}
\newcommand{\bDv}{\ensuremath{\mathbf{\undertilde{\bD}}}}
\newcommand{\bPv}{\ensuremath{\mathbf{\undertilde{\bP}}}}
\newcommand{\Uv}{\ensuremath{\undertilde{U}}}
\newcommand{\bUv}{\ensuremath{\mathbf{\undertilde{\bU}}}}
\newcommand{\bUva}{\ensuremath{\mathbf{\undertilde{\bUa}}}}
\newcommand{\bLvah}{\ensuremath{\mathbf{\undertilde{\bLah}}}}
\newcommand{\bVv}{\ensuremath{\mathbf{\undertilde{\bV}}}}
\newcommand{\bSigmav}{\ensuremath{\mathbf{\undertilde{\bSigma}}}}
\newcommand{\sigmav}{\ensuremath{\undertilde{\sigma}}}
\newcommand{\av}{\ensuremath{\undertilde{a}}}
\newcommand{\bav}{{\ensuremath{\mathbf{\undertilde{\ba}}}}}
\newcommand{\bcv}{{\ensuremath{\mathbf{\undertilde{\bc}}}}}
\newcommand{\bdv}{{\ensuremath{\mathbf{\undertilde{\bd}}}}}
\newcommand{\bnv}{{\ensuremath{\mathbf{\undertilde{\bn}}}}}
\newcommand{\bsv}{{\ensuremath{\mathbf{\undertilde{\bs}}}}}


\newcommand{\Uav}{\ensuremath{\undertilde{\Ua}}}
\newcommand{\bUav}{\ensuremath{\mathbf{\undertilde{\bUa}}}}
\newcommand{\bAcv}{\ensuremath{\mathbf{\undertilde{\bAc}}}}
\newcommand{\bncv}{\ensuremath{\mathbf{\undertilde{\bnc}}}}
\newcommand{\bscv}{\ensuremath{\mathbf{\undertilde{\bsc}}}}

\newcommand{\Pap}{\bPv_{\bA}^\perp}
\newcommand{\Papt}{\bPv_{\bA(\sbtheta)}^\perp}

\def\bones{{\bf 1}}
\def\bzero{{\bf 0}}

\def\circone{
    {\ooalign{
   \smash{\hskip3.0pt\raise0pt\hbox{\small $1$}}\vphantom{}\crcr
   \hbox{$\bigcirc$}
	}}
	} 
\def\circtwo{
    {\ooalign{
   \smash{\hskip3.0pt\raise0pt\hbox{\small $2$}}\vphantom{}\crcr
   \hbox{$\bigcirc$}
	}}
	} 
\def\circthree{
    {\ooalign{
   \smash{\hskip3.0pt\raise0pt\hbox{\small $3$}}\vphantom{}\crcr
   \hbox{$\bigcirc$}
	}}
	} 

\newcommand{\Xap}{\Xa^{+}}
\newcommand{\Yap}{\Ya^{+}}

\newcommand{\Xd}{X^{\dagger}}
\newcommand{\Xdd}{X^{\ddagger}}
\newcommand{\Wd}{W^{\dagger}}
\newcommand{\Wdd}{W^{\ddagger}}
\newcommand{\Ld}{L^{\dagger}}

\newcommand{\Gi}{\Gamma^{-\!1}}
\newcommand{\Yi}{Y_{[i]}}
\newcommand{\Ui}{U_{[i]}}
\newcommand{\Zi}{Z^{-\!1}}

\newcommand{\Xk}{X_{[k]}}
\newcommand{\Yk}{Y_{[k]}}
\newcommand{\Uk}{U_{[k]}}

\newcommand{\ET}{\tilde{E}_T}
\newcommand{\HT}{\tilde{H}_T}
\newcommand{\KT}{\tilde{K}_T}
\newcommand{\KTr}{\tilde{K}_{Tr}}
\newcommand{\TT}{\tilde{T}_T}
\newcommand{\VT}{\tilde{V}_T}
\newcommand{\Hu}{\HT^{\scriptstyle \uparrow}}
\newcommand{\Hl}{\HT^{\scriptstyle \leftarrow}}
\newcommand{\LmZi}{\cL^m Z^{-\!1}}

\newcommand{\bXh}{{\hat{\bX}}}
\newcommand{\cHh}{{\hat{\cH}}}
\newcommand{\bQh}{{\hat{\bQ}}}

 

%  []
% \def\qed{\hfill {$\Box$}}
% The tex-book p.106: adapted `signed' macro to ensure qed always at end of line
\def\qed{{\unskip\nobreak\hfil\penalty50
    \hskip2em\hbox{}\nobreak\hfil{$\Box$}
    \parfillskip=0pt \vspace{2ex}\par}}

\newcommand{\nsimeq}{\stackrel { N}{\simeq} }

\newcommand{\sqperp}{^{[\perp]}}
\newcommand{\sqperpto}{{\mathbin{\;[\perp]\;}}}
%  [+] and [-]
\def\sqplus{\mathbin{
	{\ooalign{\hfil\raise.3ex\hbox{\scriptsize
	+}\hfil\crcr\mathhexbox274\crcr\mathhexbox275}}
	}} 
\def\sqminus{\mathbin{
	{\ooalign{\hfil\raise.3ex\hbox{\scriptsize
	--}\hfil\crcr\mathhexbox274\crcr\mathhexbox275}}
	}} 



% The set of complex numbers
\def\IC{{
   \mathord{
      \hbox to 0em{
	 \hskip-4pt
         \ooalign{
	   \smash{\hskip1.9pt\raise2.6pt\hbox{$\scriptscriptstyle |$}}\crcr
	   \smash{\hbox{\rm\sf C}} }
	 \hidewidth}
      \phantom{\hbox{\rm\sf C}}
} }}
% The set of natural numbers
\def\IN{
    {\ooalign{
   \smash{\hskip2.2pt\raise1.5pt\hbox{$\scriptscriptstyle |$}}\vphantom{}\crcr
   \hbox{\sf N}
	}}
	} 
% The set of integers
\def\IZ{
    {\ooalign{
   \smash{\hskip1.9pt\raise0pt\hbox{$\sf Z$}}\vphantom{}\crcr
   \hbox{\sf Z}
	}}
	} 
% The set of reals
\def\IR{
    {\ooalign{
   \smash{\hskip2.2pt\raise1.5pt\hbox{$\scriptscriptstyle |$}}\vphantom{}\crcr
   \smash{\hskip2.2pt\raise3.3pt\hbox{$\scriptscriptstyle |$}}\vphantom{}\crcr
   \hbox{\sf R}
	}}
	} 

% hacks for bold \Sigma and \Theta in TimesRoman: 
\def\boldgreek#1{{
      \ooalign{
	\smash{\hskip.3pt\raise.1pt\hbox{$#1$}}\vphantom{}\crcr
	\smash{\hskip.5pt\raise.2pt\hbox{$#1$}}\vphantom{}\crcr
	\hbox{$#1$}\vphantom{$#1$}}}}
	%\smash{\hbox{$#1$}}\vphantom{$#1$}}}}

\iffalse
    % use definition from ams (doesn't work with times+m)
    \usepackage{amsbsy}
    \newcommand{\bSigma}{{\ensuremath{\boldsymbol{\Sigma}}}}
    \newcommand{\blambda}{{\ensuremath{\boldsymbol{\lambda}}}}
    \newcommand{\bLambda}{{\ensuremath{\boldsymbol{\Lambda}}}}
    \newcommand{\bGamma}{{\ensuremath{\boldsymbol{\Gamma}}}}
    \newcommand{\bPhi}{{\ensuremath{\boldsymbol{\Phi}}}}
    \newcommand{\bTheta}{{\ensuremath{\boldsymbol{\Theta}}}}
    \newcommand{\bOmega}{{\ensuremath{\boldsymbol{\Omega}}}}
    \newcommand{\btheta}{{\ensuremath{\boldsymbol{\theta}}}}
    \newcommand{\bDelta}{{\ensuremath{\boldsymbol{\Delta}}}}

    %\newcommand{\bSa}{{\ensuremath{\boldsymbol{\hat{\Sigma}}}}}

    \newcommand{\bthetaa}{{\ensuremath{\hat{\boldsymbol{\btheta}}}}}
\else
    \newcommand{\bSigma}{{\ensuremath{\boldgreek{\Sigma}}}}
    \newcommand{\blambda}{{\ensuremath{\boldgreek{\lambda}}}}
    \newcommand{\bLambda}{{\ensuremath{\boldgreek{\Lambda}}}}
    \newcommand{\bGamma}{{\ensuremath{\boldgreek{\Gamma}}}}
    \newcommand{\bPhi}{{\ensuremath{\boldgreek{\Phi}}}}
    \newcommand{\bTheta}{{\ensuremath{\boldgreek{\Theta}}}}
    \newcommand{\bOmega}{{\ensuremath{\boldgreek{\Omega}}}}
    \newcommand{\btheta}{{\ensuremath{\boldgreek{\theta}}}}
    \renewcommand{\balpha}{{\ensuremath{\boldgreek{\alpha}}}}
    \newcommand{\bDelta}{{\ensuremath{\boldgreek{\Delta}}}}

    \newcommand{\bSa}{{\ensuremath{\hat{\boldgreek{\Sigma}}}}}
    \newcommand{\bLah}{\ensuremath{\boldgreek{\hat{\Lambda}}}}

    \newcommand{\bthetaa}{{\ensuremath{\boldgreek{\hat{\theta}}}}}
    \newcommand{\sbtheta}{{\mbox{\scriptsize{$\btheta$}}}}
\fi

\def\bdot{{\scriptscriptstyle\bullet}}


% Indented 'list' 
% Usage: \SI
%          blabla
%        \EI

\def\indlist{\list{\mbox{}}{\topsep 0pt 
    \itemsep 5pt \parsep 0.3ex plus .25pt \parskip 0pt
    \labelwidth 20pt \itemindent 0pt \labelsep 2pt \listparindent 0pt
    \leftmargin 22pt }\item}
    \let\endindlist\endlist
\newcommand{\SI}{\begin{indlist}}
\newcommand{\EI}{\end{indlist}}


%
% Special list with boxes
% Usage: \begin{descr}
%        \item  blabla
%        \item  blabla
%        \end{descr}
\def\descr{\list{\mbox{$\Box$}}{\topsep 5pt plus .25pt
    \itemsep 5pt \parsep 0.3ex plus .25pt
    \labelwidth 12pt \itemindent 0pt \labelsep 3pt \listparindent 0pt
    \leftmargin 15pt }}
    \let\enddescr\endlist


% Hanging indent after introline
% usage:
%    \hanglines{where\ }
%    $U$ is block lower and unitary,\\
%    $V$ is block upper and isometric, and\\
%    $T_0$ is upper with upper inverse.
%
\def\hanglines#1{
    \setbox1=\hbox{#1}%
    \hangindent=\wd1\hangafter=0
    \hskip -\hangindent
    \makebox[\hangindent]{\box1}\ignorespaces%
}

\def\dashlist{\list{\mbox{--}}{\topsep 5pt plus .25pt
    \itemsep 5pt \parsep 0.3ex plus .25pt
    \labelwidth 12pt \itemindent 0pt \labelsep 3pt \listparindent 0pt
    \leftmargin 15pt }}
    \let\enddashlist\endlist
%
\newcommand{\DL}{\begin{dashlist}}
\newcommand{\DLE}{\end{dashlist}}

